Simplicial 2-Complex Convolutional Neural Nets

Recently, neural network architectures have been developed to accommodate when the data has the structure of a graph or, more generally, a hypergraph. While useful, graph structures can be potentially limiting. Hypergraph structures in general do not account for higher order relations between their hyperedges. Simplicial complexes offer a middle ground, with a rich theory to draw on. We develop a convolutional neural network layer on simplicial 2-complexes.

==> conclusion.tex <==
\section{Conclusion}



==> downstream_layers.tex <==
\section{Downstream layers}

In this section we briefly describe two methods
